Neural Dehydration: Effective Erasure of Black-box Watermarks from DNNs with Limited Data

To protect the intellectual property of well-trained deep neural networks (DNNs), black-box watermarks, which are embedded into the prediction behavior of DNN models on a set of specially-crafted samples and extracted from suspect models using only API access, have gained increasing popularity in both academy and industry. Watermark robustness is usually implemented against attackers who steal the protected model and obfuscate its parameters for watermark removal. However, current robustness evaluations are primarily performed under moderate attacks or unrealistic settings. Existing removal attacks could only crack a small subset of the mainstream black-box watermarks, and fall short in four key aspects: incomplete removal, reliance on prior knowledge of the watermark, performance degradation, and high dependency on data. In this paper, we propose a watermark-agnostic removal attack called \textsc{Neural Dehydration} (\textit{abbrev.} \textsc{Dehydra}), which effectively erases all ten mainstream black-box watermarks from DNNs, with only limited or even no data dependence. In general, our attack pipeline exploits the internals of the protected model to recover and unlearn the watermark message. We further design target class detection and recovered sample splitting algorithms to reduce the utility loss and achieve data-free watermark removal on five of the watermarking schemes. We conduct comprehensive evaluation of \textsc{Dehydra} against ten mainstream black-box watermarks on three benchmark datasets and DNN architectures. Compared with existing removal attacks, \textsc{Dehydra} achieves strong removal effectiveness across all the covered watermarks, preserving at least $90\%$ of the stolen model utility, under the data-limited settings, i.e., less than $2\%$ of the training data or even data-free.

==> tex/abs.tex <==
\begin{abstract}
To protect the intellectual property of well-trained deep neural networks (DNNs), black-box DNN watermarks, which are embedded into the prediction behavior of DNN models on a set of specially-crafted samples, have gained increasing popularity in both academy and industry. Watermark robustness is usually implemented against attackers who steal the protected model and obfuscate its parameters for watermark removal. Recent studies empirically prove the robustness of most black-box watermarking schemes against known removal attempts. 

In this paper, we propose a novel Model Inversion-based Removal Attack (\textsc{Mira}), which is watermark-agnostic and effective against most of mainstream black-box DNN watermarking schemes.
In general, our attack pipeline exploits the internals of the protected model to recover and unlearn the watermark message. We further design target class detection and recovered sample splitting algorithms to reduce the utility loss caused by \textsc{Mira} and achieve data-free watermark removal on half of the watermarking schemes. We conduct comprehensive evaluation of \textsc{Mira} against ten mainstream black-box watermarks on three benchmark datasets and DNN architectures. Compared with six baseline removal attacks, \textsc{Mira} achieves strong watermark removal effects on the covered watermarks, preserving  at least $90\%$ of the stolen model utility,
under more relaxed or even no assumptions on the dataset availability.
\end{abstract}


%%% Generated by Notion AI, Waiting for refinements

